Infinite Recommendation Networks: A Data-Centric Approach

We leverage the Neural Tangent Kernel and its equivalence to training infinitely-wide neural networks to devise $\infty$-AE: an autoencoder with infinitely-wide bottleneck layers. The outcome is a highly expressive yet simplistic recommendation model with a single hyper-parameter and a closed-form solution. Leveraging $\infty$-AE's simplicity, we also develop Distill-CF for synthesizing tiny, high-fidelity data summaries which distill the most important knowledge from the extremely large and sparse user-item interaction matrix for efficient and accurate subsequent data-usage like model training, inference, architecture search, etc. This takes a data-centric approach to recommendation, where we aim to improve the quality of logged user-feedback data for subsequent modeling, independent of the learning algorithm. We particularly utilize the concept of differentiable Gumbel-sampling to handle the inherent data heterogeneity, sparsity, and semi-structuredness, while being scalable to datasets with hundreds of millions of user-item interactions. Both of our proposed approaches significantly outperform their respective state-of-the-art and when used together, we observe 96-105% of $\infty$-AE's performance on the full dataset with as little as 0.1% of the original dataset size, leading us to explore the counter-intuitive question: Is more data what you need for better recommendation?

==> NeurIPS '22 -- Final/algorithms/distillation.tex <==
% \vspace{-0.1cm}
\begin{algorithm}[H]
\centering
\caption{Data synthesis using \sampler} \label{alg:distill}
    \begin{flushleft}
        \textbf{Input:} $\text{User set}~~ \mathcal{U} ~;~ \text{dataset}~ \mathbf{X} \in \mathbb{R}^{|\mathcal{U}| \times |\mathcal{I}|} ;$ NTK $\mathbb{K} : \mathbb{R}^{|\mathcal{I}|} \times \mathbb{R}^{|\mathcal{I}|} \mapsto \mathbb{R} ~;~ \text{support user size}~ \mu \in \mathbb{R} ~;~ $ \\
        gumbel softmax temperature $\tau \in \mathbb{R} ~;~ \text{reg. const.}~ \lambda_2 \in \mathbb{R} ~;~ \text{SGD batch-size}~ b, \text{step-size}~ \eta \in \mathbb{R}$ \\
        \textbf{Output:} Synthesized data $\mathbf{X^s} \in \mathbb{R}^{\mu \times |\mathcal{I}|}$
    \end{flushleft}
    \begin{algorithmic}[1]
        \Procedure{sample}{$n, \mathcal{U}, \mathbf{X}$} 
            \State $\mathcal{U}' \sim \mathcal{U}$ \Comment{Randomly sample $n$ users from $\mathcal{U}$}
            \State $\mathbf{X'} \leftarrow \mathbf{X_u} ~~~ \forall u \in \mathcal{U}'$ \Comment{Retrieve corresponding rows from $\mathbf{X}$}
            \State \Return $\mathcal{U}', \mathbf{X'}$
        \EndProcedure
    
        \Procedure{synthesize}{$\mathcal{U}, \mathbf{X}, \mathbb{K}$} 
            \State $\mathcal{U}^s, \mathbf{X^s} \leftarrow \textsc{sample}(\mu, \mathcal{U}, \mathbf{X})$ \Comment{Sample support data}
            \For{$steps = 0 \ldots \xi$}
                \State $\mathbf{\hat{X}^s} \leftarrow \sigma \left[ \sum_{i=1}^{\gamma} gumbel_{\tau}(softmax(\mathbf{X^s})) \right]$
                \State $\alpha^s \leftarrow \textsc{fit}(\mathcal{U}^s, \mathbf{\hat{X}^s}, \mathbb{K})$ 
                \Comment{Fit \model on support data}
                \State $\mathcal{U}^b, \mathbf{X^b} \leftarrow \textsc{sample}(b, \mathcal{U}, \mathbf{X})$
                \State $\mathbf{\Tilde{X}} \leftarrow [0]_{b \times |\mathcal{I}|}$
                \State $\mathbf{\Tilde{X}_u} \leftarrow \textsc{predict}(\mathcal{U}^s, \mathbf{\hat{X}^s}, \mathbf{X^b_u}, \mathbb{K}, \alpha^s) ~~~ \forall u \sim \mathcal{U}^b$ \Comment{Predict for all sampled users}
                \State $L \leftarrow \mathbf{X^b} \cdot log(\mathbf{\Tilde{X}}) + (1 - \mathbf{X^b}) \cdot log(1 - \mathbf{\Tilde{X}}) + \lambda_2 \cdot ||\mathbf{\hat{X}^s}||_1$ \Comment{Re-construction loss}
                \State $\mathbf{X^s} \leftarrow \mathbf{X^s} - \eta \cdot \dfrac{\partial L}{\partial \mathbf{X^s}}$ \Comment{SGD on $\mathbf{X^s}$}
            \EndFor
            \State \Return $\mathbf{X^s}$
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

==> NeurIPS '22 -- Final/algorithms/inf_ae_predict.tex <==
\vspace{-0.5cm}
\begin{algorithm}[H]
\centering
\caption{\model inference} \label{alg:inf_ae_predict}
    \begin{flushleft}
        \textbf{Input:} $\text{User set}~~ \mathcal{U} ~;~ \text{dataset}~ \mathbf{X} \in \mathbb{R}^{|\mathcal{U}| \times |\mathcal{I}|} ;$ NTK \\
        $\mathbb{K} : \mathbb{R}^{|\mathcal{I}|} \times \mathbb{R}^{|\mathcal{I}|} \mapsto \mathbb{R} ;~ \text{dual params.}~ \alpha \in \mathbb{R}^{|\mathcal{U}| \times |\mathcal{I}|}$ \\
        $;~ \text{inference user history}~ \hat{\mathbf{X}}_u \in \mathbb{R}^{|\mathcal{I}|} $ \\
        \textbf{Output:} $\text{Prediction}~ \hat{y} \in \mathbb{R}^{|\mathcal{I}|}$
    \end{flushleft}
    \begin{algorithmic}[1]
        \Procedure{predict}{$\mathcal{U}, \mathbf{X}, \hat{\mathbf{X}}_u, \mathbb{K}, \alpha$} 
            \State $\mathbf{K} \leftarrow [0]_{|\mathcal{U}|}$ 
            \Comment{Zero Initialization}
            \State $\mathbf{K}_{v} \leftarrow \mathbb{K}(\hat{\mathbf{X}}_u, \mathbf{X}_v) ~~~ \forall v \in \mathcal{U}$
            \State $\hat{y} \leftarrow softmax(\mathbf{K} \cdot \alpha)$
            \State \Return $\hat{y}$
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

==> NeurIPS '22 -- Final/algorithms/inf_ae_train.tex <==
\vspace{-0.5cm}
\begin{algorithm}[H]
\centering
\caption{\model model training} \label{alg:inf_ae_trian}
    \begin{flushleft}
        \textbf{Input:} $\text{User set}~~ \mathcal{U} ~;~ \text{dataset}~ \mathbf{X} \in \mathbb{R}^{|\mathcal{U}| \times |\mathcal{I}|} ;$ NTK \\
        $\mathbb{K} : \mathbb{R}^{|\mathcal{I}|} \times \mathbb{R}^{|\mathcal{I}|} \mapsto \mathbb{R} ~;~ \text{regularization const.}$ \\ $\lambda \in \mathbb{R}$ \\
        \textbf{Output:} $\text{Dual parameters}~ \alpha \in \mathbb{R}^{|\mathcal{U}| \times |\mathcal{I}|}$
    \end{flushleft}
    \vspace{0.1cm}
    \begin{algorithmic}[1]
        \Procedure{fit}{$\mathcal{U}, \mathbf{X}, \mathbb{K}$} 
            \State $\mathbf{K} \leftarrow [ 0 ]_{|\mathcal{U}| \times |\mathcal{U}|}$ 
            \Comment{Zero Initialization}
            % \For{$u \sim \mathcal{U}, v \sim \mathcal{U}$}
            \State $\mathbf{K}_{u, v} \leftarrow \mathbb{K}(\mathbf{X}_u, \mathbf{X}_v) ~~~ \forall u \in \mathcal{U}, v \in \mathcal{U}$
            % \EndFor
            \State $\alpha \leftarrow (\mathbf{K} + \lambda I)^{-1} \cdot \mathbf{X}$
            \State \Return $\alpha$
        \EndProcedure
    \end{algorithmic}
    \vspace{0.08cm}
\end{algorithm}

==> NeurIPS '22 -- Final/general_definitions.tex <==
% \makeatletter \renewcommand\paragraph{\@startsection{paragraph}{4}{\z@} {2mm \@plus1ex \@minus.2ex} {-0.7em} {\normalfont\normalsize\bfseries}} \makeatother
\makeatletter \renewcommand\paragraph{\@startsection{paragraph}{4}{\z@} {2mm \@plus1ex \@minus.2ex} {-0.7em} {\normalfont\normalsize\bfseries}} \makeatother

\newcommand{\listheader}[1]{\item \emph{#1} }

\newcommand\overstar[1]{\ThisStyle{\ensurestackMath{%
  \setbox0=\hbox{$\SavedStyle#1$}%
  \stackengine{0pt}{\copy0}{\kern.2\ht0\smash{\SavedStyle*}}{O}{c}{F}{T}{S}}}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}

\newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}

\newcommand{\bs}[1]{\ensuremath{\bm{\mathit{#1}}}}

% \newcommand{\ns}[1]{\textcolor{blue}{[Noveen: #1]}}
% \newcommand{\mehak}[1]{\textcolor{red}{[Mehak: #1]}}
% \newcommand{\jm}[1]{\textcolor{purple}{[Julian: #1]}}
\newcommand{\ie}[0]{\emph{i.e.}\xspace}
\newcommand{\etc}[0]{\emph{etc.}\xspace}
\newcommand{\eg}[0]{\emph{e.g.}\xspace}
\newcommand{\vs}[0]{\emph{vs.}\xspace}
\newcommand{\wrt}[0]{\emph{w.r.t.}\xspace}


==> NeurIPS '22 -- Final/recsys_definitions.tex <==
\newcommand{\dataset}[0]{$\mathcal{D}$\xspace}
\newcommand{\sampled}[0]{$\mathcal{D}'$\xspace}
\newcommand{\argmin}[1]{\underset{#1}{\operatorname{arg}\,\operatorname{min}}\;}
\newcommand{\expectation}[2]{\underset{#1}{\mathbb{E}} \left[#2\right]}

% \newcommand{\oracle}{\textsc{Data-genie}\xspace}
\newcommand{\sampler}{\textsc{Distill-CF}\xspace}
\newcommand{\model}{\textsc{$\infty$-AE}\xspace}
% \newcommand{\samplerprop}{\textsc{SVP-CF-Prop}\xspace}

\newcommand{\EE}{\operatornamewithlimits{\mathbb{E}}} % Expectation

==> NeurIPS '22 -- Final/tables/co2e.tex <==
\begin{table}[!t]
    \vspace{-5mm} %Put here to reduce too much white space after your table
    \caption{CO$_2$ emissions comparison \cite{co2e}}
    \label{co2e}
    \begin{footnotesize} % normalsize, small, footnotesize
    \begin{center}
        \begin{tabular}{c c}
            \toprule
            \textbf{Consumption} & \textbf{CO$_2$e (lbs.)} \\ \midrule
            
            1 person, NY$\leftrightarrow$SF flight      & 2k \\
            Human life, 1 year avg.                     & 11k \\ 
            \midrule
            Weekly RecSys development cycle             & 20k \\
            '' \ \ \ \ \emph{w/} \oracle                & 3.4k \\
            
            \bottomrule
        \end{tabular}
    \end{center}
    \end{footnotesize}
    \vspace{-2mm} %Put here to reduce too much white space after your table
\end{table}

==> NeurIPS '22 -- Final/tables/data_stats.tex <==
% \newcommand{\STAB}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}
\begin{table*}%[!ht]
    \begin{small} % scriptsize
    \caption{Brief set of statistics of the datasets used in this paper.}
    \label{data_stats}
    \begin{center}
        \begin{tabular}{c | c c c c}
            \toprule
            Dataset & \# Users & \# Items & \# Interactions & Sparsity \\
            
            \midrule
            
            % \textbf{\STAB{Amazon\\Magazine}}    & 3k & 1.3k & 12k & 99.7\% \\
            \textbf{Amazon Magazine \cite{amz_data}}            & 3k & 1.3k & 12k & 99.7\% \\
            \textbf{ML-1M \cite{movielens}}                      & 6k & 3.7k & 1M & 95.6\% \\
            \textbf{Douban \cite{douban_data}}                     & 2.6k & 34k & 1.2M & 98.7\% \\
            % \textbf{KuaiRec}                    & 7k & 10k & 12.5M & 83.8\% \\
            \textbf{Netflix \cite{netflix_data}}                    & 476k & 17k & 100M & 98.9\% \\
            
            \bottomrule
        \end{tabular}
    \end{center}
    \end{small}
\end{table*}

==> NeurIPS '22 -- Final/tables/hyper_params.tex <==
\begin{table*}%[!ht]
    \begin{small} % scriptsize
    \caption{List of all the hyper-parameters grid-searched for \model, \sampler, and baselines.}
    \label{tab:hyper_params}
    \begin{center}
        \begin{tabular}{c c | c c c c}
            \toprule
            Hyper-Parameter & Model & Amz. Magazine & ML-1M & Douban & Netflix \\
            
            \midrule
            
            \multirow{4}{*}{Latent size}    & MF        & \multicolumn{4}{c}{\multirow{4}{*}{\{4, 8, 16, 32, 50, 64, 128\}}} \\
                                            & NeuMF     & & & & \\
                                            & LightGCN  & & & & \\
                                            & MVAE      & & & & \\
            
            \midrule
            
            \multirow{5}{*}{\# Layers}      & MF        & \multicolumn{4}{c}{\multirow{4}{*}{\{1, 2, 3\}}} \\
                                            & NeuMF     & & & & \\
                                            & LightGCN  & & & & \\
                                            & MVAE      & & & & \\
                                            & \model    & \multicolumn{4}{c}{\{1\}} \\
            
            \midrule
            
            \multirow{5}{*}{Learning rate}  & MF        & \multicolumn{3}{c}{\multirow{4}{*}{\{0.001, 0.006, 0.01\}}} & \multirow{4}{*}{\{0.006\}} \\
                                            & NeuMF     & & & & \\
                                            & LightGCN  & & & & \\
                                            & MVAE      & & & & \\
                                            & \sampler  & \multicolumn{4}{c}{\{0.04\}} \\
            
            \midrule
            
            \multirow{4}{*}{Dropout}        & MF        & \multicolumn{4}{c}{\multirow{4}{*}{\{0.0, 0.3, 0.5\}}} \\
                                            & NeuMF     & & & & \\
                                            & LightGCN  & & & & \\
                                            & MVAE      & & & & \\
            
            \midrule
            
            \multirow{3}{*}{$\lambda$}      & EASE      & \multicolumn{4}{c}{\{1, 10, 100, 1K, 10K\}} \\
                                            & \model    & \multicolumn{4}{c}{\{0.0, 1.0, 5.0, 20.0 50.0, 100.0\}} \\
                                            & \sampler  & \multicolumn{4}{c}{\{1e-5, 1e-3, 0.1, 1.0, 5.0, 50.0\}} \\
            
            \midrule
            
            $\lambda_2$                     & \sampler  & \multicolumn{4}{c}{$\dfrac{\text{\{1e-3, 10.0\}}}{\text{avg. \# of interactions per user}}$} \\
            
            \midrule
            
            $\tau$                          & \sampler  & \multicolumn{4}{c}{\{0.3, 0.5, 0.7, 5.0\}} \\
            
            \midrule
            
            $\gamma$                        & \sampler  & \{50, 100, 200\} & \{200, 500, 700\} & \{500, 1K, 2K\} & \{500, 700\} \\
            
            \bottomrule
        \end{tabular}
    \end{center}
    \end{small}
\end{table*}

==> NeurIPS '22 -- Final/tables/model_results.tex <==
\newcommand{\bb}[1]{\textbf{#1}}
\newcommand{\uu}[1]{\underline{#1}}
\begin{table*}%[!ht]
    \begin{scriptsize} % scriptsize
    \caption{Comparison of \model with different methods on various datasets. All metrics are better when higher. Brief set of data statistics can be found in \cref{appendix:hyper_params}, \cref{data_stats}. \bb{Bold} values represent the best in a given row, and \uu{underlined} represent the second-best. Results for \model on the Netflix dataset (marked with a *) consist of random user-sampling with a max budget of $25$K $\equiv 5.4$\% users, and results for \sampler + \model have a user-budget of $500$ for all datasets.}
    \label{tab:results}
    \begin{center}
        \begin{tabular}{c | c | c c c c c c c | c c}
            \toprule
            \multirow{2}{*}{Dataset} & \multirow{2}{*}{Metric} & \multirow{2}{*}{PopRec} & \multirow{2}{*}{\STAB{Bias\\only}} & \multirow{2}{*}{MF} & \multirow{2}{*}{NeuMF} & \multirow{2}{*}{\STAB{Light\\GCN}} & \multirow{2}{*}{EASE} & \multirow{2}{*}{MVAE} & \multirow{2}{*}{\model} & \multirow{2}{*}{\STAB{\sampler\\+ \model}} \\
            
            & & & & & & & & & \\
            
            \midrule
            
            \multirow{6}{*}{\textbf{\STAB{Amazon\\Magazine}}} 
            & AUC       & 0.8436    & 0.8445    & 0.8475    & 0.8525    & 0.8141    & 0.6673        & 0.8507    & \uu{0.8539}   & \bb{0.8584} \\
            & HR@10     & 14.35     & 14.36     & 18.36     & 18.35     & \uu{27.12}& 26.31         & 17.94     & 27.09         & \bb{28.27} \\
            & HR@100    & 59.5      & 59.35     & 58.94     & 59.3      & 58.00     & 48.36         & 57.3      & \uu{60.86}    & \bb{61.78} \\
            & NDCG@10   & 8.42      & 8.33      & 13.1      & 13.6      & 22.57     & 22.84         & 12.18     & \uu{23.06}    & \bb{23.81} \\
            & NDCG@100  & 19.38     & 19.31     & 21.76     & 21.13     & 29.92     & 28.27         & 19.46     & \uu{30.75}    & \bb{31.75} \\
            & PSP@10    & 6.85      & 6.73      & 9.24      & 9.00      & 13.2      & 12.96         & 8.81      & \uu{13.22}    & \bb{13.76} \\
            
            \midrule
            
            \multirow{6}{*}{\textbf{ML-1M}} 
            & AUC       & 0.8332    & 0.8330    & 0.9065    & 0.9045    & 0.9289    & 0.9069    & 0.8832    & \bb{0.9457}   & \uu{0.9415} \\
            & HR@10     & 13.07     & 12.93     & 24.63     & 23.25     & 27.43     & 28.54     & 21.7      & \bb{31.51}   & \uu{31.16} \\
            & HR@100    & 30.38     & 29.63     & 53.26     & 51.42     & 55.61     & 57.28     & 52.29     & \bb{60.05}   & \uu{58.28} \\
            & NDCG@10   & 13.84     & 13.74     & 25.65     & 24.44     & 28.85     & 29.88     & 22.14     & \bb{32.82}   & \uu{32.52} \\
            & NDCG@100  & 19.49     & 19.13     & 35.62     & 33.93     & 38.29     & 40.16     & 33.82     & \bb{42.53}   & \uu{41.29} \\
            & PSP@10    & 1.10      & 1.07      & 2.41      & 2.26      & 2.72      & 3.06      & 2.42      & \bb{3.22}   & \uu{3.15} \\
            
            \midrule
            
            \multirow{6}{*}{\textbf{Douban}} 
            & AUC       & 0.8945    & 0.8932    & 0.9288    & 0.9258    & 0.9391    & 0.8570    & 0.9129    & \bb{0.9523}   & \uu{0.9510} \\
            & HR@10     & 11.06     & 10.71     & 12.69     & 12.79     & 15.98     & 17.93     & 15.36     & \bb{23.56}   & \uu{22.98} \\
            & HR@100    & 17.07     & 16.63     & 20.29     & 19.69     & 22.38     & 25.41     & 22.82     & \bb{28.37}   & \uu{27.20} \\
            & NDCG@10   & 11.63     & 11.24     & 13.21     & 13.33     & 16.68     & 19.48     & 16.17     & \bb{24.94}   & \uu{24.20} \\
            & NDCG@100  & 12.63     & 12.27     & 14.96     & 14.39     & 17.20     & 19.55     & 17.32     & \bb{23.26}   & \uu{22.21} \\
            & PSP@10    & 0.52      & 0.50      & 0.63      & 0.63      & 0.86      & 1.06      & 0.87      & \bb{1.28}   & \uu{1.24} \\
            
            \midrule
            
            % \multirow{6}{*}{\textbf{KuaiRec}} 
            % & AUC       & 0.8859    & 0.8800    & 0.9158    & 0.8832    & \multirow{6}{*}{\STAB{Timed\\Out}}    & 0.9092    & 0.9069    & \uu{0.9545}   & \uu{0.9466} \\
            % & HR@10     & 14.40     & 19.48     & 23.44     & 18.96     &     & 33.85     & 41.40     & \bb{47.68}   & \uu{42.94} \\
            % & HR@100    & 15.08     & 15.96     & 21.17     & 16.27     &     & 26.47     & 30.26     & \bb{34.67}   & \uu{32.57} \\
            % & NDCG@10   & 13.07     & 19.67     & 22.90     & 18.39     &     & 30.69     & 42.59     & \bb{49.28}   & \uu{43.84} \\
            % & NDCG@100  & 14.78     & 16.65     & 21.15     & 16.73     &     & 26.83     & 32.04     & \bb{36.86}   & \uu{34.06} \\
            % & PSP@10    & 0.68      & 0.94      & 1.13      & 0.80      &     & 1.69      & 2.07      & \bb{2.40}   & \uu{2.12} \\
            
            % \midrule
            
            \multirow{6}{*}{\textbf{Netflix}} 
            & AUC       & 0.9249    & 0.9234    & 0.9234    & 0.9244    & \multirow{6}{*}{\STAB{Timed\\Out}}   & 0.9418   & 0.9495    & \uu{0.9663}*   & \bb{0.9728} \\
            & HR@10     & 12.14     & 11.49     & 11.69     & 11.06     &    & 26.03        & 20.6     & \bb{29.69}*    & \uu{29.57} \\
            & HR@100    & 28.47     & 27.66     & 27.72     & 26.76     &    & \uu{50.35}   & 44.53    & \bb{50.88}*    & 49.24 \\
            & NDCG@10   & 12.34     & 11.72     & 12.04     & 11.48     &    & 26.83        & 20.85    & \bb{30.59}*    & \uu{30.54} \\
            & NDCG@100  & 17.79     & 16.95     & 17.17     & 16.40     &    & 35.09        & 29.22    & \bb{36.59}*    & \uu{35.58} \\
            & PSP@10    & 1.45      & 1.28      & 1.31      & 1.21      &    & 3.59         & 2.77     & \bb{3.75}*     & \uu{3.62} \\
            
            \bottomrule
        \end{tabular}
    \end{center}
    \end{scriptsize}
    % \bigskip
    % \vspace{-6mm} %Put here to reduce too much white space after your table
\end{table*}

==> tables/co2e.tex <==
\begin{table}[!t]
    \vspace{-5mm} %Put here to reduce too much white space after your table
    \caption{CO$_2$ emissions comparison \cite{co2e}}
    \label{co2e}
    \begin{footnotesize} % normalsize, small, footnotesize
    \begin{center}
        \begin{tabular}{c c}
            \toprule
            \textbf{Consumption} & \textbf{CO$_2$e (lbs.)} \\ \midrule
            
            1 person, NY$\leftrightarrow$SF flight      & 2k \\
            Human life, 1 year avg.                     & 11k \\ 
            \midrule
            Weekly RecSys development cycle             & 20k \\
            '' \ \ \ \ \emph{w/} \oracle                & 3.4k \\
            
            \bottomrule
        \end{tabular}
    \end{center}
    \end{footnotesize}
    \vspace{-2mm} %Put here to reduce too much white space after your table
\end{table}
